Deep Learning Accelerator in Loop Reliability Evaluation for Autonomous Driving

The reliability of deep learning accelerators (DLAs) used in autonomous driving systems has significant impact on the system safety. However, the DLA reliability is usually evaluated with low-level metrics like mean square errors of the output which remains rather different from the high-level metrics like total distance traveled before failure in autonomous driving. As a result, the high-level reliability metrics evaluated at the post-silicon stage may still lead to DLA design revision and result in expensive reliable DLA design iterations targeting at autonomous driving. To address the problem, we proposed a DLA-in-loop reliability evaluation platform to enable system reliability evaluation at the early DLA design stage.

==> acknowledge.tex <==
\section{Acknowledgement}\label{acknowledgement}

This work is supported in part by National Natural Science Foundation of China under Grant No.61834006 and No.61674048, Strategic Priority Research Program of Chinese Academy of Sciences under Grant No XDC05030200. The corresponding author is Cheng Liu.

==> conclusion.tex <==
\section{conclusion} \label{sec:conclusion}
The reliability of DLAs is of vital importance to the mission-critical AI applications. Prior redundancy design approaches for the regular computing array such as RR, CR and DR greatly reduce the hardware overhead compared to the classical DMR and TMR approaches, but they are rather sensitive to the fault distribution and fail to work especially when the hardware faults are not evenly distributed. To address this problem, we propose an HCA and have a DPPU to recompute all the operations mapped to the fault PEs in the 2D computing array. When the number of faulty PEs in the 2D computing array is less than the DPPU size, HCA can fully repair the 2D computing array despite the fault distribution. Even when the fault error rate further increases, DPPU can be used to repair the most critical PEs first to ensure a large continuous computing array and minimize the performance penalty. According to our experiments, HCA outperforms prior redundancy approaches in terms of fully functional probability and computing power under different fault distribution models. In addition, it also exhibits higher scalability with moderate chip area overhead.








==> motivation.tex <==
\section{Background and Motivation} \label{sec:motivation}
\subsection{Deep Learning Accelerator Architecture}
\begin{figure}
	\center{\includegraphics[width=0.8\linewidth]{figures/accelerator.pdf}}
    \caption{A typical DLA with 2D computing array architecture.}
\label{fig:accelerator}
\vspace{-1em}
\end{figure}

A typical DLA with 2D computing array is shown in Figure \ref{fig:accelerator}. The computing array is composed of multiple homogeneous connected PEs. Each PE includes a multiplier and an accumulator and can only communicate with its neighbors. Neural network operations such as convolution can be mapped to the computing array and executed in lock-step. To ensure the high-throughput processing, the input data, weights and output must be stored in on-chip buffers to avoid external memory access stalls. In this work, we adopt a widely used output stationary data flow for the deep neural network execution. Each PE is responsible for the processing of a single output feature data and PEs in the same column calculate different output feature data in the same output channel. %In this case, we need to read input feature data and weights from various locations of the on-chip buffers concurrently when they are sequentially stored in the on-chip buffers. In addition, the same data may also be loaded multiple times. Because the pattern of the weight is different from the input pattern, the two types of data are stored in the buffer in different modes. The two types of data are read into the buffer array at their own pace to complete the calculation.%While it is expensive to increase the on-chip buffer ports or duplicate the data, usually a set of register files are inserted between the weight/input buffers and the computing array to improve the data reuse and alleviate the on-chip buffer accesses. The sizes of the register files are closely related with the computing array size. In this example, suppose the data width are 8 and the array size is $32 \times 8$. The weight register file and the input register file size are set to be $16 \times 32 \times 8bit$ and $32 \times 32 \times 8bit$ respectively.

\subsection{Influence of Faulty Computing Array}
To analyze the influence of faulty computing array, we inject random bit flip errors to registers of the PEs in a $32 \times 8$ computing array. Both input feature data and weights are 8bit fixed point while the accumulator in each PE is set to be 32bit in case of computing overflow. We have a cycle-accurate DLA simulator implemented following the architecture mentioned in previous sub section for the fault analysis and run a typical digital classification task with MNIST dataset. For each bit error injection rate, we generate 50 fault configurations with different random seeds and evaluate the prediction accuracy. The experiment result is shown in Figure \ref{fig:bit}. It reveals that the prediction accuracy varies dramatically across the different fault configurations. The prediction accuracy may drop considerably even under very low error injection rate. Thereby, protecting the computing array is necessary for mission-critical applications despite the fault injection rate. 

On top of the prediction accuracy, we also evaluate the classical hardware redundancy strategies i.e. RR, CR and DR for the regular 2D computing array and measure the fully functional probability of the computing array under different PE error rate. The evaluation result is shown in Figure \ref{fig:mo}. It can be observed that these classical redundant design approaches can hardly mitigate all the faulty PEs even when the PE error rate is 1\% and the situation deteriorates with the increase of the fault injection rate, which can be rather risky for mission-critical AI applications.  


\begin{figure}
	\center{\includegraphics[width=0.9\linewidth]{figures/bit-flipping.pdf}}
    \caption{Prediction accuracy of a neural model executed on a typical DLA with different PE error rate. For each PE error rate, 50 random fault configurations are evaluated on MNIST.}
\label{fig:bit}
\vspace{-1em}
\end{figure}

\begin{figure}
	\center{\includegraphics[width=0.85\linewidth]{figures/motivation.pdf}}
    \caption{The fully functional probability of the 2D computing array under different PE error rate.}
\label{fig:mo}
\vspace{-1em}
\end{figure}



==> relatedwork.tex <==
\section{Related Work} \label{sec:relatedwork}
With the increasing adoption of deep learning in mission-critical applications, the reliability of DLAs widely utilized for the deep learning processing becomes critical and attracts a lot of attentions of the researchers recently. To analyze the influence of hardware faults on the deep neural network model, the authors in \cite{zhang2019fault} conducted comprehensive experiments and the experiment results show that hardware faults can lead to considerable prediction accuracy drop. For the TIMIT speech recognition task, the accuracy drops from 74.13$\%$ to 39.69$\%$. The accuracy loss is relevant to various design factors including the quantization, data format, and network architecture. It remains rather challenging to ensure resilient deep neural network execution on DLAs.  

To alleviate the influence of hardware faults on deep neural network prediction, many of the prior works took advantage of the inherent fault-tolerance of the deep neural network models by retraining the models for a specific fault configuration such that hardware faults can be compensated by the retrained deep learning models. Xu et.al \cite{xu2019resilient} proposed an on-accelerator retraining framework to obtain models that can tolerate the in-deterministic hardware faults. Li et. al \cite{li2019squeezing} and wang et.al \cite{wang2016frequency}\cite{wang2017resilience} proposed to employ the model retraining for DLAs with overclocking which may incur timing errors. To train resilient deep learning models, He et. al \cite{he2018joint} revised the loss function to obtain models that are less sensitive to the hardware faults. Unlike the above methods, Fukushi et. al \cite{horita2008analysis} proposed to bypass faulty PEs in the computing array with 0 or other constant values such that the faults are more easier to tolerate via retraining. Although the retraining works for many fault configurations, there is still no guarantee that the retrained models can maintain the prediction accuracy for the target mission-critical applications because of the huge number of different fault configurations. In addition, the retraining can be rather expensive especially for large datasets and models, and is required for each specific fault configuration, which further limits the adoption of the retraining approaches. 

To enable unmodified deep learning model execution without accuracy loss, an intuitive approach is to develop reliable DLA architectures with the conventional TMR and DMR approaches to tolerate the hardware faults, but these approaches incur substantial hardware resource consumption. The authors in \cite{takanami2017built}\cite{takanami2012built}\cite{takanami1995neural}\cite{horita2000fault} proposed to add redundant PEs to the large regular homogeneous computing array and each redundant PE can be shared by a group of PEs. Distinct redundancy sharing methods such as row redundancy (RR), column redundancy (CR) and diagonal redundancy (DR) have been proposed. For the RR and CR, each row/column of the PEs share the same set of redundant PEs. For the DR, both the row and column of PEs corresponding to a diagonal location in the computing array share the same set of redundant PEs. Since the redundant PEs are shared by a group of homogeneous PEs, hardware resource consumption can be greatly reduced compared to DMR and TMR. Nevertheless, the faulty PEs may not be evenly distributed or even clustered \cite{stapper1983integrated} across the computing array. As a result, these approaches may fail to recover the computing array when the number of faulty PEs in each shared region such as a row or a column of PEs exceeds the the number of shared redundant PEs in the region. Thereby, the utilization of the redundant PEs can be affected by the fault distribution dramatically. More redundant PEs must be designed to ensure reliable execution. Otherwise, the performance can degrade dramatically when the faulty PEs are discarded directly. Thereby, more efficient computing array architectures are demanded for the resilient DLA design. 

%design is required. a grid array self-reconfiguration method based on simple column bypass and southbound rerouting scheme, which combines the advantages of high probability of successful reconstruction, low hardware overhead, and simple implementation. In \cite{chuang2005efficient}, a new reconstruction scheme and reconstruction algorithm are proposed. By configuring an appropriate number of spare PEs in the best position of the network, and adding some well-connected backup links to achieve fault tolerance. Lin et al. \cite{lin2009fault} Proposed a fault-tolerant router design to reduce the impact of a faulty router in a chip multiprocessor system based on a 2d grid. Unlike redundant strategies that have spare PEs, the downgrade strategy attempts to use as many fault-free PEs as possible to construct logical sub-arrays to achieve fault tolerance. Low and Leong \cite{low1997reconfiguration} proposed an optimal algorithm Gcr based on the "greedy" strategy, which constructs a maximum target array containing the selected rows in linear time. This optimization algorithm was adopted in \cite{low2000efficient}, and an efficient heuristic reconstruction algorithm under the constraints of row and column rerouting was obtained. In \cite{jigang2009preprocessing}, a new preprocessing and partial redirection technique is proposed to accelerate the reconstruction of degradable arrays. In addition, in \cite{zhao2020algorithm}, a faulty array-based ABFT algorithm is used to detect the fault location, and a variety of checksum schemes are used to repair the erroneous data.  Inspired by the previous work, we tried to combine redundancy and degradation strategies to design a novel fault-tolerant strategy that only requires minimal modifications to the hardware to cope with multiple fault distribution models.





